Can Your Model Tell a Negation from an Implicature? Unravelling Challenges With Intent Encoders

Conversational systems often rely on embedding models for intent classification and intent clustering tasks. The advent of Large Language Models (LLMs), which enable instructional embeddings allowing one to adjust semantics over the embedding space using prompts, are being viewed as a panacea for these downstream conversational tasks. However, traditional evaluation benchmarks rely solely on task metrics that don't particularly measure gaps related to semantic understanding. Thus, we propose an intent semantic toolkit that gives a more holistic view of intent embedding models by considering three tasks -- (1) intent classification, (2) intent clustering, and (3) a novel triplet task. The triplet task gauges the model's understanding of two semantic concepts paramount in real-world conversational systems -- negation and implicature. We observe that current embedding models fare poorly in semantic understanding of these concepts. To address this, we propose a pre-training approach to improve the embedding model by leveraging augmentation with data generated by an auto-regressive model and a contrastive loss term. Our approach improves the semantic understanding of the intent embedding model on the aforementioned linguistic dimensions while slightly effecting their performance on downstream task metrics.

==> floats/tab_bin.tex <==
\begin{table}[t]
\centering
\scalebox{0.88}{
\begin{tabular}{lccc}
\specialrule{0.1em}{0.2em}{0.2em}
Model & Original & Negation & Implicature \\
\hline
paraphrase            & 77.58                                                                & 82.41                                                                & 57.34                                                                   \\
IAE                   & 86.64                                                                & 79.63                                                                & 70.11                                                                   \\
instructor-base       & 89.06                                                                & 78.40                                                                 & 67.30                                                                    \\
instructor-large      & \textbf{89.59}                                                                & \textbf{87.38}                                                                & \textbf{73.54}                                                                  \\
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{Binary classification.}
\label{tab:eval_res_bin}
\end{table}

==> floats/tab_challenges.tex <==
\begin{table*}[t]
    \centering
    \scalebox{0.90}{
    \begin{tabularx}{\textwidth}{tXXX}
        \specialrule{0.1em}{0.2em}{0.2em} \\
        Intent & Original & Negation & Implicature \\
        \hline
        check timezone & I need to know britain's timezone & I don't need to know britain's timezone & I'm not sure when to start the event in Sydney \\
        set up timer & I need to start a timer & A timer started unexpectedly & I'm planning to do my workout every day at 6 am \\
        reserve restaurant & I'd like to make a reservation at rooth chris, can you do that & I mistakenly made a reservation at rooth chris, can you cancel that & Looking for a place to celebrate my friend's birthday with a large group \\
        why wrong exchange rate for card payment & I purchased something in a foreign currency but the rate applied is wrong & I purchased something in a foreign currency and the rate applied is correct & I've been noticing some discrepancies in my international transactions \\
        \specialrule{0.1em}{0.2em}{0.2em} \\
    \end{tabularx}}
    \vspace{-3mm}
    \caption{
    Four examples of intents, corresponding original utterances conveying the intents, negation and implicature of the original utterance where current embeddings models struggle to differentiate from the original utterance.}
    \label{tab:prelim_exp}
    \vspace{-3mm}
\end{table*}
% challenges sampled from our evaluation toolkit.


==> floats/tab_class.tex <==
\begin{table}[t]
\centering
\scalebox{0.86}{
\begin{tabular}{lcccc}
\specialrule{0.1em}{0.2em}{0.2em}
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Implicature} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
                       & 0-shot       & 10-shot       & 0-shot         & 10-shot        \\
\hline
paraphrase             & 61.06        & 83.25         & 22.21          & 28.24          \\
IAE                    & 66.58        & 84.70          & 25.45          & 30.12          \\
instructor-base        & 67.48        & 85.77         & 26.18          & 30.88          \\
instructor-large       & \textbf{67.60}         & \textbf{86.20}          & \textbf{28.79}          & \textbf{34.26}         \\
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{Classification.}
\label{tab:eval_res_class}
\end{table}

==> floats/tab_clus.tex <==
\begin{table}[t]
\centering
\scalebox{0.90}{
\begin{tabular}{lcccc}
\specialrule{0.1em}{0.2em}{0.2em}
\multirow{2}{*}{Model} & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Implicature} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
                            & KM    & Agg   & KM     & Agg     \\
\hline
paraphrase                  & 81.66      & 83.53           & 57.24       & 58.84             \\
IAE                         & 83.42      & 84.70            & 58.30        & 59.85             \\
instructor-base             & 83.82      & 84.89           & 57.93       & 59.18             \\
instructor-large            & \textbf{84.34}      & \textbf{86.01}           & \textbf{59.09}       & \textbf{61.35}    \\
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{Clustering.}
\label{tab:eval_res_clus}
\end{table}

==> floats/tab_trip.tex <==
\begin{table}[t]
\centering
\scalebox{0.9}{
\begin{tabular}{lcccc}
\specialrule{0.1em}{0.2em}{0.2em}
\multirow{2}{*}{Model}     & \multicolumn{2}{c}{Original} & \multicolumn{2}{c}{Implicature} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
 & T1 & T2 & T1 & T2 \\
\hline
paraphrase       & 22.63                             & 84.76                             & \textbf{3.87}                                 & 68.92                                \\
IAE              & \textbf{24.04}                             & 84.26                             & 3.19                                 & 67.29                                \\
instructor-base  & 19.12                             & 86.09                             & 2.04                                 & 67.95                                \\
instructor-large & 23.37                             & \textbf{87.50}                              & 3.55                                 & \textbf{70.99}                         \\      
\specialrule{0.1em}{0.2em}{0.2em}
\end{tabular}
}
\caption{Triplet task.}
\label{tab:eval_res_trip}
\end{table}
